Follow the bisector: a simple method for multi-objective optimization

This study presents a novel Equiangular Direction Method (EDM) to solve a multi-objective optimization problem. We consider optimization problems, where multiple differentiable losses have to be minimized. The presented method computes descent direction in every iteration to guarantee equal relative decrease of objective functions. This descent direction is based on the normalized gradients of the individual losses. Therefore, it is appropriate to solve multi-objective optimization problems with multi-scale losses. We test the proposed method on the imbalanced classification problem and multi-task learning problem, where standard datasets are used. EDM is compared with other methods to solve these problems.

==> background.tex <==
\section{Background}
First, we briefly introduce the concept of Pareto optimality for multi-objective optimization problem and the corresponding necessary optimality condition for differentiable losses. 

\begin{definition}[Pareto optimality]
\begin{enumerate}
\item A solution $\theta'$ dominates $\theta$ for a multi-objective optimization problem, if $\mathcal{L}_i(\theta') \leq \mathcal{L}_i(\theta)$ and at least for $1$ loss the inequality is strict.
\item A solution $\theta$ is called Pareto-optimal, if there is no other solution $\theta'$ that dominates it.
\end{enumerate}
\end{definition}
Just as in the single-objective case, there is a necessary condition for the point to be Pareto-optimal, which is called \emph{Pareto stationarity}, and it is defined in terms of the individual gradients of each loss.
\begin{definition}[Pareto stationarity]
\label{harmgrad:pardef}
Given $T$ differentiable losses $\mathcal{L}_i(\theta), i = 1, \ldots, T, \quad \theta \in X \subseteq \mathbb{R}^d$, the point $\theta_*$ is called Pareto stationary, iff there exists a convex combination of gradients $g_i = \nabla \mathcal{L}(\theta_*)$ equals to zero, i.e.
\begin{equation}
\label{harmgrad:par-stationary}
\sum_{i=1}^T \alpha_i g_i = 0, \quad \text{where } \alpha_i \geq 0, \; i=1,\ldots,T,  \quad \sum_{i=1}^T \alpha_i = 1.
\end{equation}
\end{definition}

Moreover, as it was shown in \cite{desideri2012multiple}, if we choose $\alpha_k$ by minimizing the norm of the convex combination of single-task gradients in \eqref{harmgrad:par-stationary}, we get a direction that is a descent direction for all considered losses. 
